Sampling Foundational Transformer: A Theoretical Perspective

The versatility of self-attention mechanism earned transformers great success in almost all data modalities, with limitations on the quadratic complexity and difficulty of training. To apply transformers across different data modalities, practitioners have to make specific clever data-modality-dependent constructions. In this paper, we propose Sampling Foundational Transformer (SFT) that can work on multiple data modalities (e.g., point cloud, graph, and sequence) and constraints (e.g., rotational-invariant). The existence of such model is important as contemporary foundational modeling requires operability on multiple data sources. For efficiency on large number of tokens, our model relies on our context aware sampling-without-replacement mechanism for both linear asymptotic computational complexity and real inference time gain. For efficiency, we rely on our newly discovered pseudoconvex formulation of transformer layer to increase model's convergence rate. As a model working on multiple data modalities, SFT has achieved competitive results on many benchmarks, while being faster in inference, compared to other very specialized models.

==> figure/pseudocode.tex <==
import torch
import torch.nn as nn
import torch.nn.functional as F
from torch import Tensor
from layer.utils import GRSoftmax, euclidean_score, scale_dot_score, composite_score
from layer.samsa.sam import SAM
from layer.norm import BatchNormNear, SequenceFeatureNorm
from typing import List, Union, Any, Callable, Optional
from layer.utils import _get_activation_fn
import math

def pairwise_distances(x, y):
    '''
    Input: x is a BxNxd matrix
           y is an optional BxMxd matirx
    Output: dist is a BxNxM matrix where dist[i,j] is the square norm between x[i,:] and y[j,:]
            if y is not given then use 'y=x'.
    i.e. dist[i,j] = ||x[i,:]-y[j,:]||^2
    '''
    x_norm = (x**2).sum(2).unsqueeze(2)
    y_t = torch.transpose(y, 1, 2)
    y_norm = (y**2).sum(2).unsqueeze(1)

    dist = x_norm + y_norm - 2.0 * torch.bmm(x, y_t)
    return dist

def dot_product(x, y):
    return torch.bmm(x, y.transpose(1, 2)) / math.sqrt(x.shape[-1])

class relact(nn.Module):
    def __init__(self):
        super().__init__()
        self.params = nn.Parameter(torch.tensor(10.0), requires_grad=True)

    def forward(self, x):
        return torch.minimum(x, self.params)

class RelativeSAMAttention(nn.Module):
    def __init__(self, nhead, score_functions, norm=False, hard=False, drop_global_points=False):
        super().__init__()
        if hard == False:
            self.softmax = F.softmax
        else:
            self.softmax = GRSoftmax(temp=0.1, k=3)
        self.drop_global_points = drop_global_points
        self.n_global_points = None
        self.score_functions = score_functions(norm, nhead)
        self.linear_b = nn.LazyLinear(nhead)
        self.linear_w = nn.LazyLinear(nhead)
        self.relact_b = relact()
        self.relact_w = relact()
        self.norm = BatchNormNear(1)
        
    def forward(self, q, k, v, c, d_q, d_k, mask=None, e=1e-12):
        # input is 4 dimension tensor
        # [batch_size, head, length, d_tensor]
        if d_q.shape[2] == 4:
            distmap = self.norm(pairwise_distances(d_q[:,:,:3], d_k[:,:,:3]).unsqueeze(-1))
            dotmap = dot_product(d_q[:,:,-1].unsqueeze(-1), d_k[:,:,-1].unsqueeze(-1)).unsqueeze(-1).permute(0, 3, 1, 2)
            # distmap_w = F.softplus(self.relact_w(self.linear_w(distmap)).permute(0, 3, 1, 2)) * dotmap
            distmap_w = F.sigmoid(self.linear_w(distmap).permute(0, 3, 1, 2)) * dotmap
            distmap_w = distmap_w + torch.ones_like(distmap_w) * (1 - dotmap)
            distmap_b = self.relact_b(self.linear_b(distmap)).permute(0, 3, 1, 2) * dotmap
        else:
            distmap1 = self.norm(pairwise_distances(d_q[:,:,:3], d_k[:,:,:3]).unsqueeze(-1))
            distmap2 = dot_product(d_q[:,:,3:6], d_k[:,:,3:6]).unsqueeze(-1)
            distmap = torch.cat([distmap1, distmap2], dim=-1)
            dotmap = dot_product(d_q[:,:,-1].unsqueeze(-1), d_k[:,:,-1].unsqueeze(-1)).unsqueeze(-1).permute(0, 3, 1, 2)
            distmap_w = F.softplus(self.relact_w(self.linear_w(distmap)).permute(0, 3, 1, 2)) * dotmap
            distmap_w = distmap_w + (1 - dotmap)
            distmap_b = self.relact_b(self.linear_b(distmap)).permute(0, 3, 1, 2) * dotmap
        scores = self.score_functions(q, k)
        scores = scores * distmap_w + distmap_b
        scores = F.relu(scores)
        detr = torch.sum(scores, dim=-1, keepdim=True) + torch.sum(F.softplus(c), dim=2, keepdim=True) + 1e-9
        scores = scores / detr
        v = scores @ v

        if self.drop_global_points is True:
            if self.n_global_points is None:
                self.n_global_points = int(d_q.shape[1] - torch.sum(d_q[0,:,-1]).item())
            v = v[:, :, :d_q.shape[1] - self.n_global_points, :]
        return v, scores

class RelativeSAMCMultiHeadAttention(nn.Module):
    def __init__(self, d_model, n_head, score_functions, score_norm=False, transformation_qk=True, transformation_v=True, add_zero_attn=False, hard=False, drop_global_points=False):
        super().__init__()
        self.n_head = n_head
        self.attention = RelativeSAMAttention(n_head, score_functions, score_norm, hard, drop_global_points)
        
        self.w_c = nn.Linear(d_model, n_head)

        if transformation_qk == True:
            self.w_q = nn.Linear(d_model, n_head)
            self.w_k = nn.Linear(d_model, n_head)
            self.w_v = nn.Linear(d_model, d_model)
        else:
            self.w_q = nn.Identity()
            self.w_k = nn.Identity()
            self.w_v = nn.Identity()

        if transformation_v == True:
            self.w_concat = nn.Linear(d_model, d_model)
        else:
            self.w_concat = nn.Identity()

        self.add_zero_attn = add_zero_attn
        self.d_model = d_model
        
    def forward(self, q, k, v, d_q, d_k, mask=None):
        if self.add_zero_attn == True:
            zeros = torch.zeros(k.shape[0], 1, self.d_model, device=q.device)
            k = torch.cat([k, zeros], dim=1)
            v = torch.cat([v, zeros], dim=1)

        # 1. dot product with weight matrices
        q, k, v, c = self.w_q(q), self.w_k(k), self.w_v(v), self.w_c(v)

        # 2. split tensor by number of heads
        q, k, v, c = self.split(q), self.split(k), self.split(v), self.split(c)

        # 3. do scale euclidean attention to compute similarity
        out, attention = self.attention(q, k, v, c, d_q, d_k, mask=mask)

        # 4. concat and pass to linear layer
        out = self.concat(out)
        out = self.w_concat(out)

        return out, attention

    def split(self, tensor):
        """
        split tensor by number of head

        :param tensor: [batch_size, length, d_model]
        :return: [batch_size, head, length, d_tensor]
        """
        batch_size, length, d_model = tensor.size()

        d_tensor = d_model // self.n_head
        tensor = tensor.view(batch_size, length, self.n_head, d_tensor).transpose(1, 2)
        # it is similar with group convolution (split by number of heads)

        return tensor

    def concat(self, tensor):
        """
        inverse function of self.split(tensor : torch.Tensor)

        :param tensor: [batch_size, head, length, d_tensor]
        :return: [batch_size, length, d_model]
        """
        batch_size, head, length, d_tensor = tensor.size()
        d_model = head * d_tensor

        tensor = tensor.transpose(1, 2).contiguous().view(batch_size, length, d_model)
        return tensor

class RelativeSAMMultiHeadAttention(nn.Module):
    def __init__(self, d_model, n_head, 
                 n_sampled_points_lb, n_sampled_points_ub, drop_point, drop_global_points,
                 score_functions, add_zero_attn=False, transformation_qk=True, 
                 score_norm=False, hard=False):
        super().__init__()

        self.SAM = SAM(n_sampled_points_lb, n_sampled_points_ub, d_model, drop_point)

        self.att = RelativeSAMCMultiHeadAttention(d_model, 
                                       n_head, 
                                       score_functions=score_functions,
                                       transformation_qk=transformation_qk, 
                                       add_zero_attn=add_zero_attn,
                                       hard=hard,
                                       score_norm=score_norm,
                                       drop_global_points=drop_global_points)
        
        self.d_model = d_model
        
    def forward(self, q, k, v, d_q, mask=None):
        vdq = torch.cat([v, d_q], dim=-1)
        kvdq = self.SAM(k, vdq, mask=mask)
        k, v, d_k = kvdq[:,:,:self.d_model], kvdq[:,:,self.d_model:2*self.d_model], kvdq[:,:,2*self.d_model:]
        out, attention = self.att(q, k, v, d_q, d_k, None)
        return out, attention
    
class RelativeEuclideanSAMMultiHeadAttention(nn.Module):
    def __init__(self, d_model, n_head, 
                 n_sampled_points_lb, n_sampled_points_ub, drop_point, drop_global_points,
                 add_zero_attn=False, hard=False):
        super().__init__()
        self.att = RelativeSAMMultiHeadAttention(d_model, 
                                         n_head, 
                                         n_sampled_points_lb,
                                         n_sampled_points_ub,
                                         drop_point,
                                         drop_global_points=drop_global_points,
                                         score_functions=euclidean_score, 
                                         score_norm=True, 
                                         transformation_qk=True, 
                                         add_zero_attn=add_zero_attn,
                                         hard=hard)
        
    def forward(self, q, k, v, d_q, mask=None):
        out, attention = self.att(q, k, v, d_q, mask)
        return out, attention
    
class RelativeScaledDotSAMMultiHeadAttention(nn.Module):
    def __init__(self, d_model, n_head, 
                 n_sampled_points_lb, n_sampled_points_ub, drop_point, drop_global_points,
                 add_zero_attn=False, hard=False):
        super().__init__()
        self.att = RelativeSAMMultiHeadAttention(d_model, 
                                         n_head, 
                                         n_sampled_points_lb,
                                         n_sampled_points_ub,
                                         drop_point,
                                         drop_global_points=drop_global_points,
                                         score_functions=scale_dot_score, 
                                         score_norm=False, 
                                         transformation_qk=True, 
                                         add_zero_attn=add_zero_attn,
                                         hard=hard)
        
    def forward(self, q, k, v, d_q, mask=None):
        out, attention = self.att(q, k, v, d_q, mask)
        return out, attention
    
class RelativeCompositeSAMMultiHeadAttention(nn.Module):
    def __init__(self, d_model, n_head, 
                 n_sampled_points_lb, n_sampled_points_ub, drop_point, drop_global_points,
                 add_zero_attn=False, hard=False):
        super().__init__()
        self.att = RelativeSAMMultiHeadAttention(d_model, 
                                         n_head, 
                                         n_sampled_points_lb,
                                         n_sampled_points_ub,
                                         drop_point,
                                         drop_global_points=drop_global_points,
                                         score_functions=composite_score, 
                                         score_norm=False, 
                                         transformation_qk=True, 
                                         add_zero_attn=add_zero_attn,
                                         hard=hard)
        
    def forward(self, q, k, v, d_q, mask=None):
        out, attention = self.att(q, k, v, d_q, mask)
        return out, attention
    
class RelativeNeuralSAMMultiHeadAttention(nn.Module):
    def __init__(self, d_model, n_head, 
                 n_sampled_points_lb, n_sampled_points_ub, drop_point, drop_global_points,
                 add_zero_attn=False, hard=False):
        super().__init__()
        self.att = RelativeSAMMultiHeadAttention(d_model, 
                                         n_head, 
                                         n_sampled_points_lb,
                                         n_sampled_points_ub,
                                         drop_point,
                                         drop_global_points=drop_global_points,
                                         score_functions='neural', 
                                         score_norm=False, 
                                         transformation_qk=True, 
                                         add_zero_attn=add_zero_attn,
                                         hard=hard)
        
    def forward(self, q, k, v, d_q, mask=None):
        out, attention = self.att(q, k, v, d_q, mask)
        return out, attention

==> texts/psd_kernel.tex <==
\subsection{Our attention is a PSD kernel}

A kernel $k: \mathcal{X} \times \mathcal{X} \rightarrow \mathbb{R}$ is fundamentally a function that measures the similarity between any pair of inputs $x$ and $x'$ in the input space $\mathcal{X}$. A kernel must be symmetric such that $k(x, x') = k(x', x)$. A symmetric matrix $M \in \mathbb{R}^{n \times n}$ is positive semi-definite (PSD) if $c^T M c$ is non-negative for every vector $c \in \mathbb{R}^n$. A Gram matrix, sometimes called kernel matrix, $G \in \mathbb{R}^{n \times n}$ with respect to a dataset of $n$ examples $\mathcal{D} = \{x_1, x_2, \ldots, x_n\}$, where $G_{ij} = k(x_i, x_j)$ must be positive semi-definite. Mercer's condition states that a kernel $k(\cdot, \cdot)$ must satisfy the PSD condition for any dataset of any size. In this section, theorem \ref{theorem:psd} proves that our proposed attention score function with the softsign activation, defined as $\phi_{ss}(x) = \frac{x}{1 + |x|}$, is a PSD kernel, i.e. satisfying the Mercer's condition.

\begin{theorem}\label{theorem:psd}
The attention score $k: \mathbb{R}^d \times \mathbb{R}^d \rightarrow \mathbb{R}^d$ defined as $k(x, y) = \phi_{ss}(x)^T \phi_{ss}(y)$ is a PSD kernel.
\end{theorem}

\begin{proof}
Suppose we are given a dataset $\mathcal{D} = \{x_1, x_2, \ldots, x_n\}$ of $n$ samples in which $x_i \in \mathbb{R}^d$. We construct the gram kernel matrix $G \in \mathbb{R}^{n \times n}$ so that 
$$G_{ij} = k(x_i, x_j) = \phi_{ss}(x_i)^T \phi_{ss}(x_j) = \sum_{a = 1}^d \frac{x_{ia}}{1 + |x_{ia}|} \cdot \frac{x_{ja}}{1 + |x_{ja}|}.$$
For every $c \in \mathbb{R}^n$, we have:
\begin{align}
c^T G c &= \sum_{i = 1}^n \sum_{j = 1}^n c_i c_j G_{ij} \\
&= \sum_{i = 1}^n \sum_{j = 1}^n c_i c_j \sum_{a = 1}^d \frac{x_{ia}}{1 + |x_{ia}|} \cdot \frac{x_{ja}}{1 + |x_{ja}|} \\
&= \sum_{a = 1}^d \bigg( \sum_{i = 1}^n c_i \frac{x_{ia}}{1 + |x_{ia}|} \bigg) \bigg( \sum_{j = 1}^n c_j \frac{x_{ja}}{1 + |x_{ja}|} \bigg)
\end{align}
Let
$$z_a = \sum_{i = 1}^n c_i \frac{x_{ia}}{1 + |x_{ia}|},$$
we have:
$$c^T G c = \sum_{a = 1}^d z_a^2 \geq 0.$$
Therefore, $k(\cdot, \cdot)$ is a PSD kernel.
\end{proof}
